Relat\'orio T\'ecnico: Controle Distribu\'ido de Tr\'afego Baseado em Ve\'iculos Conectados e Comunica\c{c}\~oes Veiculares Centradas em Interesses

Although advanced traffic management systems can deal with the heterogeneous traffic flows approaching of intersections, their performances are compromised, when the traffic volume is not distributed uniformly. To evenly distribute the traffic flow, an advanced driver information system should be aware of the traffic control operations. However, such requirement can not ultimately be satisfied due to the gaps in state of the art in advanced traffic management systems. Therefore, this study proposes a distributed traffic control system, in which agents embedded in connected vehicles, traffic signals, urban elements and a traffic control center interact with each other to provide a greater traffic fluidity. Therefore, the agents depend strongly on a heterogeneous vehicular network. In this sense, this study also proposes a heterogeneous vehicular network whose communication protocol can satisfy the communication requirements of intelligent transportation systems service applications. According to the results obtained from simulations, the distributed traffic control system was able to maximize the flow of vehicles and the mean speed of the vehicles, and minimize the wait time, travel time, fuel consume and emissions (CO, CO$_2$, HC, NOx and PMx).

==> dedic.tex <==
\dedication{À minha Aline, com amor.}

==> thanks.tex <==
\chapter*{Agradecimentos}

Muitas são as pessoas a quem devo agradecer por esta conquista, pois acredito que a
gratidão é uma virtude. Assim, mesmo correndo o risco de esquecer alguém, não posso deixar
de citar alguns nomes e expressar a minha eterna gratidão, são eles:

\begin{itemize}
\item A Deus, o autor e consumador da minha fé. Muito obrigado pela força para
chegar até o fim, pela sabedoria para as escolhas certas, pelo auxílio das
pessoas que você colocou no meu caminho para me ajudar e, por fim, por
estar ao meu lado em todos os momentos;
\item Aos meus pais, que foram grandes auxiliadores durante de minha vida, enquanto estudante graduação e, em seguida, mestrado;
\item A minha amada, Aline, que me entende, batalha comigo e é participante de
minhas vitórias. Te amo.
\item Aos Professores Felipe Maia Galvão França e Cláudio Luis de Amorim, um imenso muito obrigado, por acreditar em mim e por toda a compreensão e paciência que tiveram para comigo. 
 \item Aos meus tios Antônio Carlos e Gessiléia, a minha prima Vanessa e seu marido
Marcelo, por facilitarem a minha estada no Rio de Janeiro durante o período
em precisei. Sem o apoio de vocês não seria possível ter começado este
sonho;
\item Ao CNPq por ter financiado esta tese, oferecendo suporte financeiro na forma de bolsa de estudos. 

\end{itemize}

